UniCAIM: A Unified CAM/CIM Architecture with Static-Dynamic KV Cache Pruning for Efficient Long-Context LLM Inference

Transformer-based large language models (LLMs) have achieved impressive performance in various natural language processing (NLP) applications. However, the high memory and computation cost induced by the KV cache limits the inference efficiency, especially for long input sequences. Compute-in-memory (CIM)-based accelerators have been proposed for LLM acceleration with KV cache pruning. However, as existing accelerators only support static pruning with a fixed pattern or dynamic pruning with primitive implementations, they suffer from either high accuracy degradation or low efficiency. In this paper, we propose a ferroelectric FET (FeFET)-based unified content addressable memory (CAM) and CIM architecture, dubbed as UniCAIM. UniCAIM features simultaneous support for static and dynamic pruning with 3 computation modes: 1) in the CAM mode, UniCAIM enables approximate similarity measurement in O(1) time for dynamic KV cache pruning with high energy efficiency; 2) in the charge-domain CIM mode, static pruning can be supported based on accumulative similarity score, which is much more flexible compared to fixed patterns; 3) in the current-domain mode, exact attention computation can be conducted with a subset of selected KV cache. We further propose a novel CAM/CIM cell design that leverages the multi-level characteristics of FeFETs for signed multibit storage of the KV cache and in-place attention computation. With extensive experimental results, we demonstrate UniCAIM can reduce the area-energy-delay product (AEDP) by 8.2-831x over the state-ofthe-art CIM-based LLM accelerators at the circuit level, along with high accuracy comparable with dense attention at the application level, showing its great potential for efficient long-context LLM inference.

==> doc/outline.tex <==
DAC paper outline:

\begin{itemize}
    \item Introduction:
    \begin{itemize}
        \item For end-to-end stochastic computing (SC) accelerator, accumulation and non-linear functions takes the majority of the latency, area and area-delay product (ADP). With the scaling of DNNs, the accumulation and activation module becomes even more dominating. \red{@Tengyu, @Yixuan, need to show the area/ADP breakdown for both the AxPC+FSM based and BSN based accelerators.}
        \item Requirements on the accumulation and activation module: accuracy, efficiency, and flexibility
        \begin{itemize}
            \item Accuracy: fig about non-liner adder std to nn accuracy
            \item Flexibility: support different input sizes, activation functions, etc. Current design has to scale with the network.
            \item Efficiency: area-delay product.
        \end{itemize}
        \item Existing baselines, including 1) MUX + FSM, 2) APC + FSM, 3) AxPC + FSM, and 4) BSN + selective connection cannot satisfy all these requirements. \red{Are there any other baselines?}
        \begin{itemize}
            \item 1), 2), and 3) all suffer from limited accuracy for high dimensional reduction and ReLU activations. Specifically, 1) requires long BSL for accurate accumulation while 2) and 3) can only be applied to small scale networks with limited accumulation width. 
            \item 4) suffers from poor efficiency and flexibility.
        \end{itemize}
        \item \red{How to highlight our design? what is the single most important feature we want to highlight?} maybe flexibility (trade off between Accuracy-Efficiency)
    \end{itemize}
    \item Background:
    \begin{itemize}
        \item Simple introduction to the end-to-end SC accelerator architecture
        \item Requirements for accumulation + activation module, and comparison between different designs \red{Need a table here for a qualitative comparison. Need the figure on error comparison for APC/MUX + FSM and BSN + selective connection for both ReLU and Sigmoid.}
        \item Detailed introduction to BSN + selective connection: need to highlight the fully parallel architecture, which forces the BSN scale to increase with the network.
    \end{itemize}
    \item Core techniques:
    \begin{itemize}
        \item We use BSN + selective connection as the baseline and try to improve its flexibility and explore the trade-off between accuracy and efficiency.
        \item Optimization 1: approximate BSN for accuracy and efficiency trade-off
        \begin{itemize}
            \item Key observation: mis-match between output BSL and accumulation BSL
            \item Propose progressive sorting and approximation network
            \item Design parameters: num. of stages, num. of inputs, approximation parameters (including clipping factors and scaling factors)
            \item Fast design space exploration for approximate BSN
        \end{itemize}
        \item Optimization 2: time folded BSN
        \begin{itemize}
            \item Flexible support for input sizes that are not power of 2
            \item Decouple the BSN size and the network scale
        \end{itemize}
        \item Optimization 3: supporting accumulation bit widths that are not power of 2
        % \item Optimization 3: composable BSN: better support smaller number of accumulations or lower bit precision \red{Need to double check}
        % \item Optimization 1: Time-folded BSN: better support larger number of accumulations or higher bit precision.
        % \begin{itemize}
        %     \item Need to highlight 
        % \end{itemize}
        % \item Optimization 2: composable BSN: better support smaller number of accumulations or lower bit precision \red{Need to double check}
        % \item Optimization 3: accuracy and efficiency trade-off through progressive sorting + approximation
        % \begin{itemize}
        %     \item Error analysis for the accumulation
        %     \item Design space exploration
        % \end{itemize}
        % \item Optimization 4: leverage sparsity to further reduce the BSN inputs $\rightarrow$ leverage n:m sparsity \red{Any other hardware design optimization?}
    \end{itemize}
    \item Experimental results:
    \begin{itemize}
        \item Design space exploration results: Pareto front between ADP and accuracy, error plot comparison between BSN and approximate BSN
        \item Hardware: ADP, area, latency comparison, etc.
        \begin{itemize}
            \item Baseline: 1) MUX + FSM, 2) APC + FSM, 3) AxPC + FSM, 4) BSN + selective connection
        \end{itemize}
        \item Network accuracy: inject error into the network and show the accuracy comparison for important networks, e.g., ResNet, MobileNet on Cifar10, Cifar100, and TinyImagenet.
        \begin{itemize}
            \item 
        \end{itemize}
    \end{itemize}
\end{itemize}

\newpage

BSN optimization space:
\begin{itemize}
    \item Num. of inputs: $n$
    \item Num. of outputs: $m$
    \item Max num. of stages: $\log_2(n/m)$
    \item Each stage can be represented by:
    \begin{itemize}
        \item Num. of fused stages $l$
        \item Symmetric clipping factor $c$
        \item Sub-sampling factor $s$
    \end{itemize}
    \item Total num. of possibilities: 
\end{itemize}
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figs/subsample_block.pdf}
    \caption{Optimization parameter for each sub-sample block.}
    \label{fig:ss_block}
\end{figure}

Noise analysis:

\begin{itemize}
    \item Noise sources: quantization noise (can be partially compensated with QAT) and hardware approximation noise (e.g., for add and mul, hard to accurately model during training)
\end{itemize}

For simple cases, assuming we can realize round operation during subsampling.
\begin{align*}
    x_q & = \lceil x \rfloor = x + q_x \\
    y_q & = \sum_{i}^{N_x} x_q[i] + q_y = \sum_{i}^{N_x} x[i] + \sum_{i}^{N_x} q_x[i] + q_y = y + \hat{q}_y
\end{align*}
where $q_x \in [\frac{-\Delta_x}{2}, \frac{\Delta_x}{2}]$ is the quantization error. $q_y$ is the re-quantization error to convert a high precision integer to a low precision integer.

Hence, we have
\begin{align*}
    \sigma_{q_x}^2 & = \frac{\Delta_{x}^2}{12} \\
    \sigma^2_{\sum_{i}^{N_x} q_x[i]} & = N_x \sigma_{q_x}^2 \\
    % \sigma_{q_y}^2 & = \frac{\Delta_y^2}{12}
    \sigma^2_{\hat{q}_y} & = N_x \sigma_{q_x}^2 + \sigma^2_{q_y}
\end{align*}
Assuming $E[x] = 0$, i.e., $x$ is a random variable with zero mean, then, we have
\begin{align*}
    \sigma_{x}^2 = E[x^2] \\
    \sigma_{y}^2 = N_x E[x^2]
\end{align*}
Now consider the second accumulation step. We have
\begin{align*}
    z_q = \sum_{i}^{N_y}y_q[i] + q_z = \sum_{i}^{N_y} y[i] + \sum_{i}^{N_y} \hat{q}_y[i] + q_z = z + \hat{q}_z
\end{align*}
where
\begin{align*}
    \sigma^2_{\sum_{i}^{N_y} \hat{q}_y[i]} & = N_y \sigma^2_{\hat{q}_y} \\
    \sigma^2_{\hat{q}_z} & = N_x N_y \sigma^2_{q_x} + N_y \sigma^2_{q_y} + \sigma^2_{q_z} \\
    \sigma^2_{z} & = N_y \sigma^2_{y} = N_x N_y \sigma^2_{x}
\end{align*}

Following the analysis above, we can calculate the SNR for $z_q$ is
\begin{align*}
    \log \frac{\sigma^2_{z}}{\sigma^2_{\hat{q}_z}} = \log N_x N_y \sigma^2_{x} - \log (N_x N_y \sigma^2_{q_x} + N_y \sigma^2_{q_y} + \sigma^2_{q_z})
\end{align*}


\begin{figure}
    \centering
    \includegraphics[width=6cm]{figs/BSN512.png}
    \caption{16~512BSL implemented by 512-BSN and basic BSN}
    \label{fig:BSN512}
\end{figure}

\newpage
